Fact or Fiction: Verifying Scientific Claims

We introduce scientific claim verification, a new task to select abstracts from the research literature containing evidence that SUPPORTS or REFUTES a given scientific claim, and to identify rationales justifying each decision. To study this task, we construct SciFact, a dataset of 1.4K expert-written scientific claims paired with evidence-containing abstracts annotated with labels and rationales. We develop baseline models for SciFact, and demonstrate that simple domain adaptation techniques substantially improve performance compared to models trained on Wikipedia or political news. We show that our system is able to verify claims related to COVID-19 by identifying evidence from the CORD-19 corpus. Our experiments indicate that SciFact will provide a challenging testbed for the development of new systems designed to retrieve and reason over corpora containing specialized domain knowledge. Data and code for this new task are publicly available at https://github.com/allenai/scifact. A leaderboard and COVID-19 fact-checking demo are available at https://scifact.apps.allenai.org.

==> _old-01-introduction.tex <==
\section{Introduction} \label{sec:introduction}

\input{figures/teaser.tex}

\emph{Fact-checking} -- a task in which the veracity of an input \emph{claim} is verified against a corpus of documents that \emph{support} or \emph{refute} the claim -- has seen increased attention as an important research area. This attention is motivated by the proliferation of misinformation in political news, social media, and on the web \hanna{add citations}. In turn, interest in fact-checking has spurred the creation of many datasets across different domains to support research and development of automated fact-checking systems \hanna{add citations}.
Yet, to our knowledge, no such dataset exists to facilitate research on another important domain for fact-checking -- scientific literature. The ability to verify claims about scientific concepts, especially those related to biomedicine, is an important application area for fact-checking.  Furthermore, this line of research also offers a unique opportunity to explore the capabilities of modern neural models, since
successfully verifying most scientific claims requires expert background knowledge, complex language understanding, and reasoning capability, as demonstrated in Figure \ref{fig:teaser} and Table \ref{tbl:covid_example}.

% TODO(dwadden) bring back table of examples.
% \input{tables/scifact-challenges.tex}
\input{tables/covid-example.tex}

In this paper, we introduce the task of scientific fact-checking. To facilitate research on this task, we construct \ours, an expert-annotated dataset of \numclaims scientific claims accompanied by scientific abstracts that support or refute each claim, and annotated with rationales justifying each support / refute decision. To create this dataset, we use a novel annotation protocol where annotators re-formulate naturally occurring claims in the scientific literature -- \emph{citation sentences} or \emph{``citances''} \cite{Nakov2004CitancesC} -- into \emph{atomic scientific claims}. Using citances as a claim source expedites the annotation process compared to composing claims from scratch. This approach also ensures that the distribution of topics discussed in \ours claims matches the underlying distribution in the literature, rather than focusing on areas with which the claim-writers are most familiar. In addition, citances contain citation links to the papers likely to contain relevant evidence.

To establish performance baselines on this new task, we develop a pipeline model following the ``\bert-to-\bert'' approach from \citet{DeYoung2019ERASERAB}, which achieves strong performance on \fever.  Our model, which we call \sysname, \dw{From Sewon: What are new components compared to DeYoung? If they are mostly same as DeYoung, not sure if giving it a new name is a great idea} retrieves abstracts related to a given claim, uses a \bert-based \cite{Devlin2019BERTPO} sentence selector to identify rationale sentences, and then labels each claim as \supports, \refutes, or \notenough with respect to the claim. Our system is able to identify correctly-labeled and rationalized evidence abstracts with performance of 46.5 F1, indicating that the task is doable but leaving ample room for improvement \dw{From Bhargavi: what's an upper bound from domain experts? How can we contextualize 46 somehow?}. Despite its small size, training \sysname on \ours leads to better performance than training on fact-checking datasets constructed from Wikipedia articles \cite{Thorne2018FEVERAL} and political news \cite{Hanselowski2019ARA}. The strongest performance is achieved using a simple domain adaptation strategy, pretraining on \fever and then finetuning on \ours.

To evaluate the real-world applicability of our dataset and approach, we showcase the ability of our model to verify expert-written claims concerning the novel coronavirus COVID-19 against the newly-released CORD-19 corpus \cite{Wang2020CORD19TC}. Medical student reviewers judge the retrieved evidence to be plausible in 23 of the 36 claims.\footnote{While we find these results promising, we emphasize that our model is a research prototype and should not be used to make any medical decisions whatsoever.}

% Uncomment for camera-ready.
% Our data and models will be released publicly at \website.

==> _old-02-related-work.tex <==
\section{Related work}

We review existing fact-checking datasets. Then, we give an overview of related tasks for scientific document understanding. This work also provides a potential testbed for rationalized NLP models; see \citet{DeYoung2019ERASERAB} for an overview.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Fact checking} \label{sec:fact_checking}

\dw{Shorten} The proliferation of misinformation in politics and on the web has motivated the creation of a number of fact-checking datasets of varying size and annotation complexity. For a comprehensive overview, see \citet{Hanselowski2019ARA}. We discuss characteristics of fact-checking datasets that are relevant to our work by comparing \ours to three other large datasets annotated with sentence-level rationales: \fever \cite{Thorne2018FEVERAL}, \snopes \cite{Hanselowski2019ARA}, and Perspectrum \cite{Chen2019SeeingTF}.

\paragraph{Natural vs. synthetic.} As discussed in \citet{Hanselowski2019ARA}, \emph{natural} claims occur naturally on, for instance, political debate websites or Twitter. \snopes and Perspectrum have natural claims. \emph{Synthetic} claims are written during the construction of a fact-checking dataset by mutating a sentence from the evidence document. \fever claims are synthetic. Natural claims are more realistic, but more difficult to generate and verify. Claims in \ours are natural, since they are based on citations written by researchers about prior scientific work.

\paragraph{Factual vs. opinion-based.} The statements in \fever and \snopes are primarily factoid claims like ``\emph{Barak Obama was the $44^{th}$ President of the United States.}'' It is sensible to assign a single label indicating whether a corpus supports or refutes this claim. Claims in Perspectrum are opinions like ``\emph{Animals should have lawful rights}''. For these claims, it is inappropriate to assign a single global veracity label. Instead, individual documents agreeing or disagreeing with the claim should be identified.

Scientific claims have properties of both factoid and opinion-based claims. For example, ``\emph{The $R_0$ of the novel coronavirus is 2.5}'' makes a factual assertion, but its veracity may be the subject of active scientific research. Therefore, it is not be appropriate to assign a single truth label to this claim based on a corpus. Instead, like Perspectrum, we focus on identifying individual abstracts that support or refute a given claim.

\paragraph{Stance vs. entailment.}

\dw{Combine this with the factual vs. opinion-based section. Say we assume scientific articles do not deliberately misinform.}

The political fact-checking task is often divided into two sub-tasks \cite{derczynski-etal-2017-semeval}: \emph{stance detection} predicts the attitude of a document with respect to a claim which may be subjective and under dispute, while \emph{veracity prediction} evaluates the objective truth of the claim given that evidence documents may contain misinformation or be unreliable. For scientific fact-checking, we do not expect documents to contain deliberate misinformation, nor do we expect an abstract to express an opinionated stance. Like \fever, we focus on classifying the entailment relationship between a claim and a relevant abstract.


\input{tables/dataset-comparison.tex}

%%%%%%%%%%%%%%%%%%%%

% Old way of doing things.

% The proliferation of misinformation in politics and on the web has motivated the creation of a number of fact-checking datasets of varying size and annotation complexity. For a comprehensive overview, see \citet{Hanselowski2019ARA}. We discuss the two largest fact-checking datasets for which sentence-level rationales are available. A summary is shown in Table \ref{tbl:dataset_comparison}. In our experiments, we compare the performance of models trained on these datasets to models trained on \ours.

% \fever \cite{Thorne2018FEVERAL} is a popular fact-checking dataset featuring factoid claims based on Wikipedia articles. \fever claims are \emph{synthetic}, meaning that they were created for a fact-checking dataset by altering sentences from the document containing the evidence. The claims in \ours are \emph{natural} -- they are based on citations written by researchers about prior scientific work.

% The claims in the \snopes dataset \cite{Hanselowski2019ARA} were collected from the Snopes political fact-checking website, and verified with sentence-level rationales from news articles. \snopes is more similar to \ours because its claims occur naturally in online political discussion. However, the scientific documents in \ours present additional linguistic challenges discussed in Section \todo.

% The political fact-checking task is often divided into two sub-tasks \cite{derczynski-etal-2017-semeval}: \emph{stance detection} predicts the attitude of a document with respect to a claim which may be subjective and under dispute, while \emph{veracity prediction} evaluates the objective truth of the claim given that evidence documents may contain misinformation or be unreliable. For scientific fact-checking, we do not expect documents to contain deliberate misinformation. Like \fever, we focus on \emph{recognizing textual entailment} of the claims with respect to evidence.

% \input{tables/dataset-comparison.tex}




% The fact-checking task requires a system to verify a claim against a corpus. To verify factoid claims like ``\emph{Barak Obama was the $44^{th}$ president of the United States}'', a fact-checking system is required to output a single label indicating the claim's veracity given the corpus. The corpus \supports the claim when the claim is \emph{entailed} by a collection of sentences from the corpus. Most fact-checking datasets, including \fever and \snopes, take this approach. For opinion-based claims like ``\emph{Animals should have lawful rights}'', predicting a single label is not appropriate. Instead, the system should identify all relevant documents and label their \emph{stance} toward the claim. This is the approach used in the Perspectrum dataset \cite{Chen2019SeeingTF}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Scientific document understanding} \label{sec:scidoc}

Although there are no previously existing datasets for scientific fact-checking, a number of scientific corpora exist on related tasks in scientific document understanding.

% \hanna{Also information extraction} \hanna{We do not need to add too much details on everything here, but it is important to say why fact checking is different from other problems? esp. QA}

\paragraph{Question answering} \dw{Much shorter} The BioASQ Task B \cite{Tsatsaronis2015AnOO} dataset consists of roughly 3,000 open-domain question / answer pairs issued by medical professionals, annotated with answers from PubMed articles. The questions come in a variety of formats, including extractive, ``yes / no'', and abstractive. PubMedQA \cite{Jin2019PubMedQAAD} is a large corpus of weakly-supervised ``yes / no'' questions over PubMed abstracts. The MEDIQA 2019 shared task \cite{Abacha2019OverviewOT} presents 40,000 questions from the related domains of clinical medicine and consumer health.

\paragraph{Citation contextualization}  The goal of \emph{citation contextualization} is to identify all spans in a cited document that are relevant to a particular citation in a citing document. A corpus of 20 biomedical documents with annotated contextualized citations was released at TAC 2014\footnote{\url{https://tac.nist.gov/2014/BiomedSumm/index.html}}. While the dataset was annotated by domain experts, the average inter-annotator agreement rate on annotated spans was only 21.7\% \cite{Cohan2015MatchingCT}.

\paragraph{Evidence inference}  Also related to fact-checking is the task of biomedical \emph{evidence inference} \cite{Lehman2019InferringWM}, which involves predicting the effect of a medical intervention on a specified outcome. Evidence inference can be viewed as a special case of claim verification.

\paragraph{Scientific information extraction} \dw{Shorter} Data and models exist to extract genes, proteins, and drugs \cite{Kim2003GENIAC, Krallinger2017OverviewOT}, computer science methods \cite{Luan2018MultiTaskIO}, and PICO clinical trial tags \cite{Nye2018ACW} from research abstracts. While our work focuses on verifying claims using article text, future efforts could incorporate information from automatically-extracted knowledgebases in the claim verification process.


==> _old-04-dataset.tex <==
\section{\ours\ dataset} \label{sec:dataset}

The \ours\ dataset consists of \numclaims claims derived from \numpapers biomedical articles, along with supporting evidence, forming \todo expert-annotated claim / label / evidence sets. Sources of claim and evidence are articles from \todo journals. For evidence documents, we hand-selected a small number of high-quality journals in fields broadly considered as biomedicine. The list of journals is shown in Appendix \ref{sec:evidence_journals}. The journals range in focus from basic science (e.g. \emph{Cell}) to clinical trial reports (e.g. the \emph{BMJ}). \todoit{Mention something about structured vs. unstructured abstracts.}

\subsection{Annotators}

Since both claim-writing and evidence-finding tasks require considerable expertise, we recruited undergraduate and graduate students from life sciences departments at the University of Washington to serve as annotators. The claim-writing and evidence-finding stages of the task were performed separately to minimize cognitive load on annotators.

Annotator training took place in two stages. First, the annotators attended an in-person training session for claim writing. Then, they continued to write claims remotely, but were monitored by supervisors and asked to re-write claims that did not satisfy the goals of the task. Some claim writers, other recruited annotators, along with three scientists from the Allen Institute were then trained to provide evidence judgments. Evidence annotators were assigned claims written by someone other than themselves. \todoit{is true?} Feedback on evidence annotations was provided by supervisors, and annotators were given the opportunity to correct annotations.

\subsection{Claim annotation}

\todoit{how citation sentences are selected for rewriting}

Given a citing sentence, annotators are asked to rewrite the sentence as check-able claims. The annotator is provided the context around the citing sentence, along with the title and abstract of the source scientific article. We ask the annotator to write claims based on the primary findings discussed in the citing sentence. Each claim should be about one finding on one aspect of an entity or process. When compound statements are found in the citing sentence, annotators are asked to split the citing sentence into any number of independent claims. They were asked to skip claims that are not checkable, such as \todoit{show an example}. Variety among claim language is encouraged. For example, given a citing sentence:

\todoit{example citation sentence}

\noindent an annotator may rewrite this as \todo or \todo.

A total of \todo annotators -- \todo undergraduate and \todo graduate students -- wrote claims. The most claims written by a single annotator were \todo. In initial experiments, annotators exhibited high agreement (\todo in deciding which claims to skip and which to re-write into claims.)

\subsection{Evidence annotation}

\kyle{here}

Different annotators are then tasked to determine the availability of evidence for each claim. Given a claim and the abstract of the cited article, annotators are asked to select all \textbf{evidence sets} from the abstract text. Each evidence set is a collection of one or more sentences that provide evidence in support of or contradicting the claim. The level of support is represented by a \textbf{stance label}, selected from among the options: \textsc{FullSupport}, \textsc{PartialSupport}, \textsc{PartialRefute}, and \textsc{FullRefute}. Multiple evidence sets can exist for a given claim and they do not have to share the same label. If the abstract does not provide evidence supporting or refuting the claim, annotators select \textsc{NoEvidence}.

As in \citet{Hanselowski2019ARA}, we provide more granular support / contradiction labels. These granular labels allow us to address some of the challenges of scientific fact checking described in Section \ref{sec:challenges}, such as identifying cases of missing qualifiers and/or mechanistic detail.

% \dw{Note that we're not the first ones to do partial support / contradiction; \cite{Hanselowski2019ARA} use a scale of false, mostly false, other, mostly true, true.}

Each sentence in an evidence set is then assigned a \textbf{discourse role}: \textsc{Primary} or \textsc{Background}.  A \textsc{Primary} sentence is required to derive the stance label of the evidence set -- that is, if removed, the evidence set no longer provides support or contradiction for the main body of the claim. Each evidence set must therefore contain at least one \textsc{Primary} sentence. Sentences that are not selected into any evidence set are considered \textsc{Inconclusive}.

\todoit{Example here}.

If an evidence set offers partial support or refutation towards the claim, we ask annotators to provide a rationale to the incompleteness in the form of a \textbf{claim edit}. If \textsc{PartialSupport} is selected, we ask for the claim to be edited (with minimal additions and deletions) until the selected evidence set fully supports the edited claim. If \textsc{PartialRefute} is selected, we correspondingly ask for the claim to be edited until the selected evidence set offers full refutation. For example, \todoit{add example}.

\todoit{merge this example into section \ref{sec:challenges}}
We also ask annotators to consider the specificity of support provided by the evidence. Consider the claim \textit{Smoking causes cancer}. The following annotations show evidence that is more specific and more general to the claim, and the appropriate level of support offered.

\begin{itemize}
    \item Evidence more specific than claim $\to$ \mbox{\textsc{FullSupport}}
    \begin{itemize}
        \item \textit{Smoking cigarettes} causes cancer
        \item Smoking \textit{accelerates} cancer
        \item Smoking causes \textit{lung cancer}
    \end{itemize}

    \item Evidence more general than claim $\to$ \mbox{\textsc{PartialSupport}}
    \begin{itemize}
        \item \textit{Drugs} cause cancer
        \item Smoking \textit{is associated with} cancer
        \item Smoking causes \textit{disease}
    \end{itemize}
\end{itemize}
\kyle{Check whether this is in \fever}
% This asymmetry requires a fact checker to understand general-specific relationships between entities or relations in the claim and evidence.

A total of \todo undergraduates, \todo graduate students, and three scientists at the Allen Institute annotated evidence. Of the student annotators, \todo had previously worked as claim writers. Annotators were shown a claim, and an abstract, and asked to identify all evidence sets that provide support or refutation for the claim \todoit{Show a picture of the interface}.

To measure inter-annotator agreement, \todo claim / evidence pairs were annotated by two annotators. We compute Cohen's $\kappa$ for coarse-grained and fine-grained label agreement, shown in Table \todo. We also compute sentence-level Cohen's $\kappa$ for evidence agreement, as shown in Table \todo. Finally, for comparison with retrieval models, we compute precision, recall, and F1 by  treating one  annotator's evidence as ``gold'' and the other's as ``predicted''. These results are shown in Table \todo.


\begin{itemize}
    \item \kyle{how many claims have  0, 1, 2, 3 evidence sets?}
    \item \kyle{On average, what percentage of the abstract is included in an evidence set (and broken into \textsc{Primary} and \textsc{Background}).}
    \item All unselected sentences are considered \textsc{Inconclusive}. \kyle{Can we justify why didnt separate into RelatedButInconclusive vs Unrelated?  I think compelling argument is the full abstract is almost surely related}
\end{itemize}

% \todoit{move up a section}
% \paragraph{Acronyms, aliases, and synonyms}   Acronyms (e.g. ``Human immunodeficiency virus'' and ``HIV''), aliases (e.g. ``Trastuzumab'' and ``Herceptin''), and synonyms (e.g. ``\kyle{example}'') do not warrant a \textsc{PartialSupport}.
% \kyle{Can we count how many times this occurs?}


\subsection{Dataset statistics}

Figure \todo shows the distribution of abstract lengths (in sentences) for the evidence documents. Statistics for structured and unstructured abstracts are shown separately. Figure \todo shows the distribution of stance labels. Figure \todo shows the distribution of the number of evidence sets per claim, and Figure \todo shows the distribution of the number of sentences per evidence set. The majority of supported claims are supported by a single evidence set, which usually consists of a single primary sentence.

==> _old-06-experiments.tex <==
\section{Experiments}

In our experiments, we (1) establish a performance baseline on \ours using \sysname, (2) analyze the performance of the three components of \sysname, (3) demonstrate the importance of in-domain training data, and (4) present promising qualitative results on verifying claims about COVID-19 using \sysname.

\subsection{Results}

Table \ref{tbl:main_results} shows the full-pipeline performance of \sysname on the \ours test set, evaluated using the abstract-level and sentence-level metrics defined in \S\ref{sec:task_definition}. The \fonecoarse value of 46.5 indicates that, for roughly half of the claim-abstract pairs, \sysname correctly identifies the \supports or \refutes label \emph{and} provides reasonable evidence to justify the decision. Given the difficulty of the task and limited in-domain training data, we consider this a promising result, while leaving plenty of room for improvement.

\input{tables/new-results.tex}

\paragraph{Oracle experiments} To examine the performance of each system component, we run the \sysname pipeline, replacing some components with ``oracles'' that always make correct predictions when given correct inputs.\footnote{For instance, the ``Label'' oracle always predicts the correct label as long as it is provided with at least one full gold rationale as input.} The oracles are only used for prediction; they do not affect the training process. The first three rows in Table~\ref{tbl:main_results} are \emph{double-oracle}. These experiments isolate the performance of a single model component. Row 1 shows that the retrieval module has an abstract recall of 68.5 F1. The precision is 100 because the oracle label predictor will always predict \notenough for false positive retrievals. Row 2 shows that, given gold abstracts, the rationale selection module identifies rationale sentences with an F1 of 75.4. Row 3 shows that, given gold rationales from gold abstracts, the label classifier has a label prediction F1 of 83.3. Since the test set is balanced and gold abstracts are provided, this is roughly comparable to a classification accuracy over the \supports and \refutes label classes.

The next three rows are \emph{single-oracle}. Row 4 shows the performance of the rationale selector and label classifier together, when given gold documents as input. This is similar to the \eraser evaluation setup.

\paragraph{Training datasets} During model development, we train the \componenttwo and \componentthree modules on four different datasets: \fever, \snopes, \ours, and \fever pretraining followed by \ours fine-tuning. The \componenttwo module is evaluated on its ability to identify rationale sentences given gold abstracts.\footnote{Our \fever-trained \componenttwo module achieves 79.9 sentence-level F1 on the \fever test set, virtually identical to the value of 79.6 reported in \citet{DeYoung2019ERASERAB}}. As in Section \ref{sec:evaluation}, a rationale sentence is only identified correctly if all other sentences from its gold rationale are also identified. The \componentthree module is evaluated on its classification accuracy given gold rationales from evidence abstracts (including evidence documents labeled \notenough). The results of these experiments are shown in Table \ref{tbl:components}. For \componenttwo, training on \ours alone produces good results, perhaps because domain-specific lexical cues are sufficient in most cases for identifying rationale sentences. For the more complex reasoning involved in \componentthree, domain adaptation was the most effective approach, training first on the large \fever dataset and then the smaller in-domain \ours training set. Based on these results, we use the \componenttwo module trained on \ours only, and the \componentthree module trained on \fever + \ours for our final end-to-end system \sysname. Additional implementation details can be found in Appendix \ref{sec:model_details}.

\input{tables/components.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Verifying claims about COVID-19}

We conduct exploratory experiments using our system to fact-check claims concerning COVID-19. We task a medical student to write 36 COVID-related claims. For each claim $c$, we use \sysname to predict evidence abstracts $\Ehat(c)$. The same medical student annotator assigns a label to each $(c, \Ehat(c))$ pair. A pair is labeled \emph{plausible} if at least half of the evidence abstracts in $\Ehat(c)$ are judged to have reasonable rationales and labels. It is labeled \emph{missed} if $\Ehat(c) = \emptyset$. Finally, it is labeled \emph{implausible} if the majority of the abstracts in $\Ehat(c)$ have irrelevant rationales or incorrect labels.

Table \ref{tbl:covid_example} shows two example claims, both with supporting and refuting evidence identified by \sysname. For the majority of these COVID-related claims (23 out of 36), the rationales produced by \sysname was deemed \emph{plausible} by our annotator, demonstrating that \sysname is able to successfully retrieve and classify evidence in many cases. An examination of errors reveals that the system can be confused by context, where abstracts are labeled \supports or \refutes even though the rationale sentences reference a different disease or drug from the claim. An example of this is also provided in Table \ref{tbl:covid_example}.

\input{08-discussion.tex}


==> _old-08-discussion.tex <==
\subsection{Analyses and Discussions}
\hanna{In this section you might want to discuss some qualitative results and error analyses; For example, Rationales requiring background knowledge can be part of error analyses. Do not frame this as a future direction because it sells the work as it is in progress. }
Our exploration into scientific claim verification has revealed a number of promising future research directions to improve data collection, modeling, and integration with complementary tools for scientific literature.

%%%%%%%%%%%%%%%%%%%%

\paragraph{Partial evidence}

In Figure \ref{fig:partial}, the abstract contains evidence relevant to the given claim, but the context is different (mouse vs. human). In pilot experiments, we instructed annotators to label cases of context mismatch as \spart / \rpart, and to \emph{edit} the given claim such that the evidence matched context of edited claim (see \citet{Min2020AmbigQAAA} for a related approach applied to information-seeking questions). Unfortunately, inter-annotator label agreement was only \labelkappafine Cohen's $\kappa$ due to disagreement over the \ppartial label. We hope to refine the annotation task and improve annotator agreement in the future.

\input{figures/partial.tex}

%%%%%%%%%%%%%%%%%%%%

\paragraph{Rationales requiring background knowledge}

In principle, a rationale should provide standalone justification for a model's prediction. But what if the rationale relies on the context established by the rest of the document, or never stated explicitly at all? For instance, the rationale excerpted in Figure \ref{fig:teaser} never mentions that Citalopram is an antidepressant, but this fact is required to justify the model's decision. Future work could explore integrating external knowledge sources like  \emph{abstractive rationales} which summarize the context or background knowledge necessary for a claim to follow from a given \emph{extractive} rationale.

%%%%%%%%%%%%%%%%%%%%

\paragraph{Evidence credibility and synthesis}

The system developed in this work identifies linguistic relationships between claim and evidence, but does not attempt to assess the credibility of the evidence itself.



Our system could be fruitfully combined with tools like the recently-created Scite.AI platform\footnote{https://www.scite.ai}, which assesses the strength of the results reported in a scientific article by examining the \emph{intent} of citations citing this article. In addition, claim verification systems could serve as a component in automated evidence synthesis frameworks (\S\ref{sec:related_work}), which could weight individual \supports\ / \refutes labels by the strength of their evidence documents to arrive at a corpus-level verdict.

%%%%%%%%%%%%%%%%%%%%


==> _old-10-abductive-reasoning.tex <==



We argue that scientific fact checking requires a form of abductive reasoning beyond traditional textual entailment.



==> figures/frac-abstract-rationale.tex <==
\begin{figure}[H]
  \centering
  \includegraphics[width=\columnwidth]{figures/frac-abstract-rationale-fig.pdf}

  \caption{Distribution showing the fraction of each abstract (in sentences) that is part of a rationale.}
  \label{fig:frac_abstract_rationale}
\end{figure}

==> figures/negation.tex <==
\begin{figure}[t]
  \centering

  \includegraphics[width=\columnwidth]{figures/negation-fig.pdf}
  \caption{A rationale that \supports one claim and \refutes another. The red claim was created by negating the meaning of the blue claim.}
  \label{fig:negation}
\end{figure}


==> figures/partial.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{figures/partial-fig.pdf}

  \caption{An abstract that partially supports a claim. The edited claim is fully supported.}
  \label{fig:partial}
\end{figure}

==> figures/rationale-stats.tex <==
\begin{figure}[H]
  \begin{subfigure}[t]{\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{figures/n-rationales.pdf}
  \caption{The number of rationales supporting each claim. For instance, roughly 150 unstructured abstracts contain 2 rationales.}
  \label{fig:n_rationales}
  \end{subfigure}

  % Largely redundant.
  % \begin{subfigure}[t]{\columnwidth}
  %   \centering
  %   \includegraphics[width=\columnwidth]{figures/total-sentences.pdf}
  %   \caption{The total number of sentences supporting each claim.}
  % \end{subfigure}

  \begin{subfigure}[t]{\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/rationale-length.pdf}
    \caption{The number of sentences per rationale.}
    \label{fig:rationale_length}
  \end{subfigure}

  \label{fig:rationale_stats}
  \caption{Statistics on rationales. Most claims are supported by a single rationale, but structured abstracts are more likely to have two rationales. The great majority of rationales are a single sentence.}
\end{figure}

==> scratchpad.tex <==
% Collection of random stuff we might want later.


\klcomment{feels like appendix content}
While estimating source trustworthiness has seen more attention in fake news identification \cite{baly-etal-2018-predicting}, some have shown it to also be useful in fact-checking, especially in web and social media domains \cite{Popat2017WhereTT,Nguyen2018AnIJ}.  Like \fever and \snopes, \ours does not explicitly handle this as our sources of documents are peer-reviewed academic journals.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \paragraph{Statistics}

% \kyle{Stopped here;  Need more info about train-dev-test splits for full corpus not just claim-abstract pairs} \dw{The corpus isn't split.}

% We divide the collection of claim-abstract pairs into standard train-dev-test splits.  
% The label distribution is shown in Table \ref{tbl:claim_counts}. 
% % \footnote{The test set is balanced, but the dev set is not; due to the smaller size of our dataset, we want to make sure our models have as many \refutes labels to train on as possible.} 

% Some of these medical journals feature \emph{structured} abstracts, which are organized into sections focusing on background, methods, results, and conclusions. The majority of abstracts are \emph{unstructured}. As shown in Table \ref{tbl:dataset_overview}, structured abstracts are generally longer and more likely to contain multiple rationales. The majority of claims have evidence in just a single document. 

% \input{tables/claim-counts.tex}

% For detailed dataset statistics, see Appendix \ref{sec:corpus_stats}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Label agreement

Treating the first annotator's label as gold and the second as a prediction, the label classification accuracy is \labelhumanacc. \kyle{what does this tell us that Cohen's doesn't?}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% BioMedSumm

This represents a substantial improvement over the BioMedSumm citation contextualization dataset, for which the inter-annotator agreement in selection rationale sentences is 0.27 Fleiss' $\kappa$\footnote{BioMedSumm rationales are annotated at the span level; we convert to sentence-level }

==> tables/claim-counts.tex <==
\begin{table}[t]
  \setlength{\tabcolsep}{.25em}
  \footnotesize
  \centering

  \begin{tabular}{L{0.12\linewidth} C{0.19\linewidth} C{0.19\linewidth} C{0.19\linewidth} C{0.15\linewidth}}
    \toprule
    Fold &  \supports &  \textsc{NEI} &  \refutes &   All \\
    \midrule
    Train &       332 &              304 &      173 &   809 \\
    Dev   &       124 &              112 &       64 &   300 \\
    Test  &       100 &              100 &      100 &   300 \\
    \midrule
    All   &       556 &              516 &      337 &  1409 \\
    \bottomrule
  \end{tabular}

  \caption{Distribution of claim / cited abstract labels by train-dev-test split in \ours. \textsc{NEI} stands for \notenough.}
  \label{tbl:claim_counts}
  
\end{table}


==> tables/dataset-overview.tex <==
\begin{table}[H]
  \setlength{\tabcolsep}{.25em}
  \footnotesize
  \centering

  \begin{tabular}{ l  r  r }
    \toprule
                                  & Unstructured & Structured \\
    \midrule
    \# evidence abstracts         & 340          & 146        \\
    Abstract length (median)      & 7            & 13         \\
    Number of rationales (mean) & 1.53            & 1.89          \\
    Rationale fraction (median)   & 0.14         & 0.17       \\
    \bottomrule
  \end{tabular}

  \caption{Summary statistics on the abstracts in the corpus. The \emph{Abstract length} is measured in number of sentences. The \emph{Rationale fraction} is the fraction of sentences in each abstract that are rationales.}
  \label{tbl:dataset_overview}
\end{table}

==> tables/error-analysis-old.tex <==
\begin{table*}[t]
  \setlength{\tabcolsep}{2pt}
  \footnotesize
  \centering
  \begin{tabular}{L{0.12\linewidth} L{0.33\linewidth} L{0.44\linewidth} R{0.06\linewidth} }
    \toprule
    \textbf{Mistake type} &  \textbf{Claim} &  \textbf{Gold evidence} & \textbf{Count} \\
    \thinmid

    Science background & Rapamycin accelerates aging in fruit flies. & \refutesCovid{\dots feeding rapamycin to adult Drosophila produces life span extension \dots} & 29 / 37  \\
    \hdashline[0.4pt/2pt]

    Directionality & Inhibiting glucose-6-phospate dehydrogenase impairs lipogenesis & \supportsCovid{\dots suppression of 6PGD decreased lipogenesis \dots} & 9 / 37 \\

    \hdashline[0.4pt/2pt]

    Numerical reasoning & Bariatric surgery reduces resolution of diabetes. & \refutesCovid{Strong associations were found \dots with a HR of 9.29 (95\% CI 6.84-12.62)...} & 9 / 37 \\

    \hdashline[0.4pt/2pt]

    Cause and effect & Major vault protein (MVP) functions to decrease tumor aggression. & \refutesCovid{Knockout of MVP leads to miR-193a accumulation...inhibiting tumor progression} & 7 / 37  \\

    \hdashline[0.4pt/2pt]

    Coreference & Low saturated fat diets have adverse effects on the development of infants & \refutesCovid{Neurological development of children in the intervention group was at least as good as ... the control group} & 6 / 37 \\

    \arrayrulecolor{black}
    \bottomrule
  \end{tabular}
  \caption{Types of reasoning required to correct 37 mistaken predictions.}
  \label{tbl:error_analysis}

\end{table*}

==> tables/n-evidence-docs.tex <==
\begin{table}[H]
  \centering
  \csvreader[autobooktabular, separator=tab, table head=\toprule\ \# evidence abstracts & Count \\ \midrule ] {tables/n-evidence-docs.tsv}{index=\ix, 0=\data}{\ix & \data}
  \caption{The number of evidence documents supporting each claim. For instance, 37 claims are supported by 2 documents.}
  \label{tbl:n_evidence_docs}
\end{table}

==> tables/old/ablations-entailment.tex <==
\begin{table}[t]
  \footnotesize
  \setlength{\tabcolsep}{0.4em}
  \centering

  \begin{subtable}{0.45\linewidth}
    \centering
    \begin{tabularx}{\columnwidth}{l r}
      \toprule
      \multicolumn{2}{r}{Label accuracy} \\
      \midrule
      \scibert   & 74.3 \\
      \bioroberta   & 76.3 \\
      \robertabase   & 72.3 \\
      \robertalarge   & 81.3 \\
      \bottomrule
    \end{tabularx}
    \subcaption{Entailment label accuracy of \bert variants.}
    \label{tbl:ablations_entailment_bert}
  \end{subtable}
  \hspace{0.2em}
  \begin{subtable}{0.45\linewidth}
    \centering
    \begin{tabularx}{\columnwidth}{l r}
      \toprule
      \multicolumn{2}{r}{Label accuracy} \\
      \midrule
      \fever   & 68.0 \\
      \snopes   & 71.7 \\
      \ours   & 76.7 \\
      \fever + \ours   & 81.3 \\
      \bottomrule
    \end{tabularx}
    \subcaption{\robertalarge trained on four different datasets.}
    \label{tbl:ablations_entailment_dataset}
  \end{subtable}

  \caption{Comparison of training procedures and \bert modules on entailment labeling.}
  \label{tbl:ablations_entailment}

\end{table}

==> tables/old/ablations-rationale.tex <==
\begin{table}[t]
  \footnotesize
  \setlength{\tabcolsep}{0.4em}
  \centering


  \begin{subtable}[h]{\linewidth}
    \begin{tabularx}{\columnwidth}{l *{3}{c}  *{3}{c}}
      \toprule
 & \multicolumn{3}{c}{\textbf{Top-$k$}} & \multicolumn{3}{c}{\textbf{Threshold}} \\
      \cmidrule(lr){2-4} \cmidrule(lr){5-7}

 & P & R & F1 & P & R & F1 \\
      \midrule
      \scibert      &       47.0 &    80.6 & 59.4 &       74.5 &    74.3 & 74.4 \\
      \bioroberta   &       47.8 &    82.0 & 60.4 &       75.3 &    69.9 & 72.5 \\
      \robertabase  &       47.5 &    81.4 & 60.0 &       76.1 &    66.1 & 70.8 \\
      \robertalarge &       48.8 &    83.6 & 61.6 &       73.7 &    70.5 & 72.1 \\
      \bottomrule
    \end{tabularx}
    \subcaption{Comparison of different \bert variants for rationale selection. All models trained on \ours.}
    \label{tbl:ablations_rationale_bert}
  \end{subtable}


  \begin{subtable}[h]{\linewidth}
    \begin{tabularx}{\columnwidth}{l *{3}{c}  *{3}{c}}
      \toprule
      & \multicolumn{3}{c}{\textbf{Top-$k$}} & \multicolumn{3}{c}{\textbf{Threshold}} \\
      \cmidrule(lr){2-4} \cmidrule(lr){5-7}

      & P & R & F1 & P & R & F1 \\
      \midrule

      \fever        &       37.6 &    64.5 & 47.5 &       65.9 &    22.1 & 33.1 \\
      \snopes       &       38.0 &    65.0 & 47.9 &       26.7 &    87.7 & 40.9 \\
      \ours         &       48.8 &    83.6 & 61.6 &       73.7 &    70.5 & 72.1 \\
      \fever + \ours &       47.5 &    81.4 & 60.0 &       72.4 &    67.2 & 69.7 \\

      \bottomrule
    \end{tabularx}
    \subcaption{Comparison of \robertalarge trained on different training datasets for rationale selection.}
    \label{tbl:ablations_rationale_dataset}
  \end{subtable}

  \caption{Comparison of training procedures and \bert modules on rationale selection.}

  \label{tbl:ablations_rationale}

\end{table}

==> tables/old/analysis-bert.tex <==
\begin{table}[t]
  \footnotesize
  \setlength{\tabcolsep}{0.4em}
  \centering

    \begin{tabularx}{\columnwidth}{l *{3}{c}  *{3}{c}}
      \toprule
      & \multicolumn{3}{c}{\textbf{Rationale selection}} & \multicolumn{3}{c}{\textbf{Entailment}} \\
      \cmidrule(lr){2-4} \cmidrule(lr){5-7}

      & P & R & F1 & \multicolumn{3}{c}{Accuracy} \\
      \midrule
      \scibert      &       47.0 &    80.6 & 59.4 &     \multicolumn{3}{c}{74.3} \\
      \bioroberta   &       47.8 &    82.0 & 60.4 &    \multicolumn{3}{c}{76.3}   \\
      \robertabase  &       47.5 &    81.4 & 60.0 &  \multicolumn{3}{c}{72.3}     \\
      \robertalarge &       48.8 &    83.6 & 61.6 &   \multicolumn{3}{c}{81.3}    \\
      \bottomrule
    \end{tabularx}

    \caption{Comparison of different \bert variants for rationale selection and entailment prediction, with gold inputs. \dw{Note that we're doing top-$k$ decoding.}}
    \label{tbl:analysis_bert}
  \end{table}

==> tables/old/compare_datasets.tex <==
\begin{table}[ht]
  \footnotesize
  \begin{tabular}{lllll}
    \hline
    & $n$ & domain     &     & rationales \\ \hline
    \fever \cite{Thorne2018FEVERAL}   &     & Wikipedia  & yes & no             \\ \hline
    \ours &     & Biomedical & yes & yes            \\ \hline
  \end{tabular}
  \caption{hi}
\end{table}

==> tables/old/covid-stats.tex <==
\begin{table}[t]
  \setlength{\tabcolsep}{.25em}
  \footnotesize
  \centering

  \begin{tabular}{ l r r r }
    \toprule
              & Plausible & Missed & Implausible \\
    \midrule
    Top-$k$   & 23        & 6      & 7           \\
    Threshold & 21        & 10     & 5           \\

    \bottomrule
  \end{tabular}

  \caption{Results returned. The majority of the results are plausible for both top-$k$ and threshold selection.}
  \label{tbl:covid_stats}
\end{table}


==> tables/old/dataset-comparison.tex <==
\begin{table}[t]
  \setlength{\tabcolsep}{.25em}
  \footnotesize
  \centering

    \begin{tabular}{ l  r  r  r }
      \toprule
      Dataset & \# Claims & Domain & Claim type \\
      \midrule
      \fever      & 185,445   & Wikipedia articles     & Synthetic             \\
      \snopes   & 6,422   & Political news      & Natural             \\
      \ours  & \numclaims  & Scientific text      & Natural             \\
      \bottomrule
    \end{tabular}

  \caption{Large fact-checking datasets annotated with rationale sentences. \dw{If keeping changes, add Perspectrum.}}
  \label{tbl:dataset_comparison}

\end{table}


==> tables/old/document-retrieval.tex <==
\begin{table}[t]
  \setlength{\tabcolsep}{.25em}
  \footnotesize

  \begin{tabular}{ l  r  r  r }
    \toprule
                     & MRR  & Retrieved One & Retrieved All \\
    \midrule
    TF-IDF & \todo & 0.89          & 0.87          \\

    \bottomrule
  \end{tabular}

  \caption{Dev set document retrieval performance. MRR is mean reciperocal rank. ``Retrieved One'' / ``Retrieved All'' are the fraction of claims for which one / all relevant abstracts were retrieved. Claims with no evidence abstracts are not included in the evaluation.}
  \label{tbl:document_retrieval}
\end{table}


==> tables/old/entailment-by-class.tex <==
\begin{table}[t]
  \setlength{\tabcolsep}{.25em}
  \footnotesize
  \centering

    \begin{tabular}{ l  r  r  r r }
      \toprule
             & oracle & first & last & pipeline \\
      \midrule
      \sfull & 1.00   & 1.00  & 1.00 & 1.00     \\
      \spart & 1.00   & 1.00  & 1.00 & 1.00     \\
      \notenough  & 1.00   & 1.00  & 1.00 & 1.00     \\
      \rpart & 1.00   & 1.00  & 1.00 & 1.00     \\
      \rfull & 1.00   & 1.00  & 1.00 & 1.00     \\
      \bottomrule
    \end{tabular}
\caption{F1 for each support, for the best-performing entailment model}

\label{tbl:entailment_by_class}

\end{table}

==> tables/old/entailment-models.tex <==
\begin{table}[t]
  \setlength{\tabcolsep}{.25em}
  \footnotesize
  \centering

  \begin{subtable}[h]{\linewidth}
    \begin{tabular}{ l  r  r  r  r }
      \toprule
                    & \fever & Snopes & \ours & \textsc{F + S} \\
      \midrule
      \scibert      & 0.52   & -      & 0.66  & 0.68           \\
      \bioroberta   & 0.48   & -      & 0.69  & 0.73           \\
      \robertabase  & 0.54   & -      & 0.56  & 0.69           \\
      \robertalarge & 0.65   & 0.66   & 0.72  & \textbf{0.80}  \\
    \end{tabular}
    \subcaption{Label macro-F1 on \ours.}
  \end{subtable}

  \caption{\Entailment prediction performance given gold rationales, measured by dev set macro-F1.}
  \label{tbl:entailment_models}

\end{table}


==> tables/old/fever-claim-types.tex <==
\begin{table}[t]
  \setlength{\tabcolsep}{.25em}
  \footnotesize
  \centering

  \begin{tabular}{ l l }
    \toprule
    \textbf{Category} & \textbf{Claim} \\
    \midrule
    is-a  & Jack Reacher is a romantic comedy.      \\
    event  & Lionel Messi was born on June 25th, 1987. \\
    part-of & New Girl has Zooey Deschanel on the cast.      \\
    aspect-of & Ireland is surrounded by ocean. \\
    \bottomrule
  \end{tabular}

  \caption{Common claim types in \fever.}
  \label{tbl:fever_claim_types}
\end{table}

==> tables/old/main-results.tex <==
\begin{table}[t]
  \footnotesize
  \setlength{\tabcolsep}{0.5em}
  \centering

  \begin{tabularx}{\linewidth}{l *{3}{c} *{1}{c} *{3}{c}}
    \toprule
    & \multicolumn{3}{c}{\textbf{Sentence-level}} & & \multicolumn{3}{c}{\textbf{Abstract-level}} \\
    \cmidrule(lr){2-4} \cmidrule(lr){6-8}

     & P & R & F1 & & P & R & F1 \\
    \midrule
    \multicolumn{3}{l}{\textbf{Oracle experiments}} \\
    \arrayrulecolor{black!30}\midrule

    \abst            &     100.0 &   68.1 & 81.0 &        &     100.0 &   68.5 & 81.3 \\
    \rtnl            &      75.1 &   75.7 & 75.4 &        &     100.0 &   84.2 & 91.4 \\
    \lbl             &      89.6 &   72.2 & 79.9 &        &      90.1 &   77.5 & 83.3 \\

    % \hdashline[0.2pt/0.4pt]\noalign{\vskip 0.6ex}
    \arrayrulecolor{black!30}\midrule

    \rtnl, \lbl      &      66.5 &   55.7 & 60.6 &        &      84.9 &   63.5 & 72.7 \\
    \abst, \lbl      &      87.6 &   49.5 & 63.2 &        &      88.9 &   54.1 & 67.2 \\
    \abst, \rtnl     &      73.5 &   54.6 & 62.6 &        &     100.0 &   59.9 & 74.9 \\


% Dropping this for arXiv.
    % \arrayrulecolor{black}\midrule
    % \multicolumn{3}{l}{\textbf{(b) Training datasets}} \\
    % \arrayrulecolor{black!30}\midrule

    % \fever       &      23.7 &   31.1 & 26.9 &        &      53.6 &   40.5 & 46.2 \\
    % \snopes      &      15.0 &   28.4 & 19.6 &        &      30.5 &   37.4 & 33.6 \\

    \arrayrulecolor{black}\midrule
    \multicolumn{3}{l}{\textbf{Final system}} \\
    \arrayrulecolor{black!30}\midrule

    \sysname         &      38.6 &   40.5 & 39.5 &        &      46.6 &   46.4 & 46.5 \\

    \arrayrulecolor{black}\bottomrule
  \end{tabularx}

    \caption{Test set performance of our \sysname system on \ours. Overall performance of our best \sysname model in \emph{Final system}. In \emph{Oracle experiments}, the three stages of the modeling pipeline are shorted to ``\abst'' for \componentone, ``\rtnl'' for \componenttwo, and ``\lbl'' for \componentthree. Each row lists the stages of the pipeline that are performed by the \sysname model. Components that are \emph{not} listed are replaced by oracles, which always make correct predictions given correct inputs. For example, the row titled ``\abst, \lbl'' uses \sysname components for abstract retrieval and label prediction, and uses an oracle for rationale selection     }
    \label{tbl:main_results}


\end{table}


==> tables/old/pipeline-components.tex <==
\begin{table}[t]
  \footnotesize
  \setlength{\tabcolsep}{0.6em}
  \centering

  \begin{tabularx}{\linewidth}{*{3}{c} *{3}{c}}
    \toprule
    & & & \multicolumn{3}{c}{\textbf{Fine-grained}} \\
    \multicolumn{3}{c}{\textbf{Oracle component}} & \multicolumn{3}{c}{Threshold decoding} \\

    \cmidrule(lr){4-6}

    Abstract & Rationale & Label & P & R & F1 \\

    \midrule

           &  $\bullet$ &  $\bullet$ &          100.0 &        68.1 &    81.0 \\
 $\bullet$ &            &  $\bullet$ &           75.1 &        75.7 &    75.4 \\
 $\bullet$ &  $\bullet$ &            &           89.6 &        72.2 &    79.9 \\
 
 \midrule
 
 $\bullet$ &            &            &           66.5 &        55.7 &    60.6 \\
           &  $\bullet$ &            &           87.6 &        49.5 &    63.2 \\
           &            &  $\bullet$ &           73.5 &        54.6 &    62.6 \\
           
          \midrule 
           
           &            &            &           38.6 &        40.5 &    39.5 \\



    \bottomrule

  \end{tabularx}
  \caption{Oracle ablations of individual pipeline components. In each row, components marked with a $\bullet$ are replaced by oracles. The first three lines show results with two oracles, isolating the performance of a single \sysname component. The next three show results with a single oracle. The last line shows the full \sysname system. \dw{Abstract retrieval, rationale selection, label prediction. Add coarse-grained too. Don't show decoding.}}
  \label{tbl:pipeline_components}



\end{table}



\begin{table}[t]
  \footnotesize
  \setlength{\tabcolsep}{0.6em}
  \centering

  \begin{tabularx}{\linewidth}{ l*{3}{c}}
    \toprule
   & \multicolumn{3}{c}{\textbf{Fine-grained}} \\
    % & \multicolumn{3}{c}{Threshold decoding} \\
   \cmidrule(lr){4-6}  & P & R & F1 \\
    \midrule 
    \multicolumn{7}{c}{Oracle Experiments} \\
      $\textsc{TFIDF}_{abst}$ + $\textsc{Oracle}_{Ratio,Label}$    &     100.0 &        68.1 &    81.0\\
   $\sysname_{Ratio}$ + $\textsc{Oracle}_{ Abst, Label}$  &           75.1 &        75.7 &    75.4 \\
   $\sysname_{Label} + \textsc{Oracle}_{Abst, Rational}$         &           89.6 &        72.2 &    79.9 \\
    \midrule
   \sysname_{ratio,Label}+\textsc{Oracle}_{Abst}   &           66.1 &        54.9 &    60.0 \\
  \sysname_{ abst, Label}+\textsc{Oracle}_{Ratio}   &           86.0 &        38.1 &    52.8 \\
  \sysname_{abst, Ratio}+\textsc{Oracle}_{Label} &           73.5 &        54.6 &    62.6 \\
    \midrule
   \multicolumn{7}{c}{Varying Training Datasets} \\
    \sysname_{FEVER}  &           40.2 &        35.1 &    37.5 \\
    \sysname_{UKP-SNOPES}  &           40.2 &        35.1 &    37.5 \\
    \sysname  &           40.2 &        35.1 &    37.5 \\
    \bottomrule
    \multicolumn{7}{c}{Varying Decoding Strategies} \\
    \sysname_{top-k}  &           40.2 &        35.1 &    37.5 \\
    \sysname_{threshold}  &           40.2 &        35.1 &    37.5 \\
   \sysname  &           40.2 &        35.1 &    37.5 \\
    \bottomrule

  \end{tabularx}
  \caption{Oracle ablations of individual pipeline components. In each row, components marked with a $\bullet$ are replaced by oracles. The first three lines show results with two oracles, isolating the performance of a single \sysname component. The next three show results with a single oracle. The last line shows the full \sysname system. \dw{Abstract retrieval, rationale selection, label prediction. Add coarse-grained too. Don't show decoding.}}
  \label{tbl:pipeline_components}



\end{table}








\begin{table}[t]
  \footnotesize
  \setlength{\tabcolsep}{0.6em}
  \centering

  \begin{tabular}{@{}lrrr}
    \toprule
   \multirow{2}{*}{Ablations} & \multicolumn{3}{c}{Fine-grained} \\
    % & \multicolumn{3}{c}{Threshold decoding} \\
   \cmidrule(lr){2-4}  & P & R & F1 \\
    \midrule 
    \multicolumn{3}{l}{\textit{Oracle components}} \\
      \hspace{1em}\textsc{tfidf }$_{\mathrm{abst}}$  &     100.0 &        68.1 &    81.0\\
   \hspace{1em}\sysname$_{\mathrm{rtnl}}$  &           75.1 &        75.7 &    75.4 \\
   \hspace{1em}\sysname$_{\mathrm{label}}$         &           89.6 &        72.2 &    79.9 \\
    \hdashline[0.2pt/0.4pt]
   \hspace{1em}\sysname$_{\mathrm{rtnl,label}}$   &           66.1 &        54.9 &    60.0 \\
  \hspace{1em}\sysname$_{\mathrm{abst, label}}$  &           86.0 &        38.1 &    52.8 \\
  \hspace{1em}\sysname$_{\mathrm{abst, rtnl}}$ &           73.5 &        54.6 &    62.6 \\
        
    \hdashline[0.2pt/0.4pt]\noalign{\vskip 0.6ex}
   \textit{Varying Training Datasets} \\
    \hspace{1em}\sysname $_\mathrm{train\:on\: \fever}$  &           40.2 &        35.1 &    37.5 \\
    \hspace{1em}\sysname $_\mathrm{train\:on\: \snopes}$  &           40.2 &        35.1 &    37.5 \\
    \hspace{1em}\sysname $_\mathrm{train\:on\: \ours}$  &           40.2 &        35.1 &    37.5 \\
        
    \hdashline[0.2pt/0.4pt]\noalign{\vskip 0.6ex}
    \textit{Varying Decoding Strategies} \\
    \hspace{1em}\sysname$_{\mathrm{top-k}}$  &           40.2 &        35.1 &    37.5 \\
    \hspace{1em}\sysname$_{\mathrm{threshold}}$  &           40.2 &        35.1 &    37.5 \\
   \hspace{1em}\sysname  &           40.2 &        35.1 &    37.5 \\
    \bottomrule

  \end{tabular}
  \caption{Oracle ablations of individual pipeline components. In each row, components marked with a $\bullet$ are replaced by oracles. The first three lines show results with two oracles, isolating the performance of a single \sysname component. The next three show results with a single oracle. The last line shows the full \sysname system. \dw{Abstract retrieval, rationale selection, label prediction. Add coarse-grained too. Don't show decoding.}}
  \label{tbl:pipeline_components}



\end{table}

==> tables/old/rationale-baselines.tex <==
\begin{table}[t]
  \setlength{\tabcolsep}{.25em}
  \footnotesize
  \centering

  \begin{tabular}{ r r r  }
    \toprule
                  first & last & tf-idf \\
    \midrule
    0.04 & 0.18 & 0.43 \\
  \end{tabular}
  \subcaption{Top-k retrieval}

  \caption{Sentence retrieval performance, measured by dev set F1. The rows of each table specify the transformer model. The columns specify the training procedure.}
  \label{tbl:rationale_baseline}

\end{table}

==> tables/old/rationale-error-analysis.tex <==
\begin{table}[t]
  \setlength{\tabcolsep}{.25em}
  \footnotesize
  \centering

  \begin{tabular}{ l  r  r  r }
    \toprule
    & Precision & Recall & F1 \\
    \midrule
    \fever top-$k$ & 0.40  & 0.68 & 0.50 \\


    \fever threshold & 0.67 & 0.22 & 0.34 \\

    \snopes top-$k$ & 0.40 & 0.68 & 0.50 \\
    \snopes threshold   & 0.27  & 0.90 & 0.42 \\

    \fever + \ours top-$k$ & 0.49 & 0.85 & 0.62 \\
    \fever + \ours threshold   & 0.75  & 0.70 & 0.73 \\
    \bottomrule
  \end{tabular}

  \caption{Threshold-based rationale retrieval performance on dev set using \robertalarge. \dw{Make this prettier}}
  \label{tbl:rationale_error_analysis}
\end{table}


==> tables/old/rationale-retrieval.tex <==
\begin{table}[t]
  \setlength{\tabcolsep}{.25em}
  \footnotesize
  \centering

%   \begin{subtable}[h]{\linewidth}
%     \begin{tabular}{ r r r  }
%       \toprule
%       first & last & TF-IDF \\
%       \midrule
%       0.04  & 0.18 & 0.43   \\
%     \end{tabular}
%     \subcaption{Top-k selection \dw{Unigram + bigram, k=3}}

%   \end{subtable}

  \begin{subtable}[h]{\linewidth}
    \begin{tabular}{ l  r r r r }
      \toprule
      Trained on    & \fever & Snopes & \ours         & \textsc{F + S} \\
      \midrule
      \scibert      & 0.54   & -      & 0.62          & 0.63           \\
      \bioroberta   & 0.47   & -      & 0.63          & 0.63           \\
      \robertabase  & 0.48   & -      & 0.63          & 0.62           \\
      \robertalarge & 0.50   & 0.50   & \textbf{0.64} & 0.62           \\
    \end{tabular}
    \subcaption{Top-k selection}
  \end{subtable}

  \begin{subtable}[h]{\linewidth}
    \begin{tabular}{ l  r r r  r}
      \toprule
                    & \fever & Snopes & \ours         & \textsc{F + S} \\
      \midrule
      \scibert      & 0.43   & -      & \textbf{0.76} & \textbf{0.76}  \\
      \bioroberta   & 0.34   & -      & 0.74          & \textbf{0.76}  \\
      \robertabase  & 0.31   & -      & 0.74          & 0.73           \\
      \robertalarge & 0.34   & 0.42   & 0.74          & 0.72           \\
    \end{tabular}
    \subcaption{Threshold selection}
  \end{subtable}

  \caption{Sentence selection performance, measured by dev set F1. The rows of each table specify the transformer model. The columns specify the training procedure. \textsc{F + S} stands for \fever + \ours.}
  \label{tbl:rationale_retrieval}

\end{table}

==> tables/scifact-challenges-old.tex <==
% Some commands for colors and symbols.

\newcommand{\lexical}[1]{{\color{c1} \textbf{#1}}}
\newcommand{\numerical}[1]{{\color{c2} \textbf{#1}}}
\newcommand{\coref}[1]{{\color{c3} \textbf{#1}}}

%%%%%%%%%%%%%%%%%%%%

\begin{table*}[t]
  \setlength{\tabcolsep}{.25em}
  \footnotesize
  \centering

  \begin{subtable}[t!]{\linewidth}
    \begin{tabularx}{\textwidth}{ X l l l }
      \toprule
      \textbf{Claim} & \textbf{Association type} & \textbf{Causal} & \textbf{Directional} \\
      \midrule
      Female carriers of the Apolipoprotein E4 (APOE4) allele have a reduced risk for Alzheimer's disease. & Mutation / Disease & \xmark & \cmark \\
      \midrule
      Side effects associated with antidepressants increases risk of mortality in postmenopausal women. & Drug / Outcome & \cmark & \cmark \\
      \midrule
      Phosphorylation of the ATM protein regulates DNA damage-induced neuronal death. & Pathway / Phenotype & \cmark & \xmark \\
      \midrule
      Tuberculosis incidence is correlated with residential crowding in the UK. & Environment / Disease & \xmark & \cmark \\
      \bottomrule
    \end{tabularx}

    \subcaption{Claims express diverse associations; some are causal and / or directional.}
    \label{tbl:scifact_claim_types}
  \end{subtable}

  %%%%%%%%%%%%%%%%%%%%

  \begin{subtable}[t]{\linewidth} 

    \begin{tabularx}{\textwidth}{ X X r }
      \toprule
      \textbf{Claim} & \textbf{Evidence} & \textbf{Label} \\
      \midrule

      Taking \lexical{antidepressants} is associated with an increase in the A$\beta$ level in the brain of experimental animals. &
      A$\beta$ production in CSF was \numerical{slowed by 37\%} in the \lexical{citalopram} group compared to placebo. &
      \refutes \\
      \midrule

      Radiographic verified pneumonia predictions are improved by the combination of physical examinations with \lexical{C-reactive protein values}. &
      Addition of \lexical{CRP} at the \numerical{optimal cut off of $>$30 mg/L} increased the \numerical{ROC area to 0.77 (0.73 to 0.81)} \dots &
      \supports \\
      \midrule

      \coref{Low saturated fat diets} do not have adverse effects on growth or development of infants. &
      Neurological development of children in the \coref{intervention group} was at least as good as that of children in the control group. &
      \supports \\
      \midrule

      \lexical{Genomic instability} in leukemia cells results from a decrease in reactive oxygen species from oncogene activation. &
      BCR/ABL-induced reactive oxygen species (ROSs) cause \lexical{chronic oxidative DNA damage} \dots &
      \refutes \\

      \bottomrule
    \end{tabularx}

    \subcaption{The fact-checking system must recognize \lexical{lexical relations}, perform \numerical{quantitative reasoning} and \coref{coreference} resolution.}
    \label{tbl:scifact_reasoning_types}
  \end{subtable}

  \caption{Examples of common challenges unique to scientific fact-checking.}
  \label{tbl:scifact_challenges}
\end{table*}


==> tables/scifact-reasoning-types.tex <==
\definecolor{c1}{rgb}{0.12, 0.46, 0.70}
\definecolor{c2}{rgb}{1.0, 0.50, 0.05}
\definecolor{c3}{rgb}{0.17,0.63,0.17}

\newcommand{\lexical}[1]{{\color{c1} \textbf{#1}}}
\newcommand{\numerical}[1]{{\color{c2} \textbf{#1}}}
\newcommand{\coref}[1]{{\color{c3} \textbf{#1}}}

\begin{table*}[t]
  \setlength{\tabcolsep}{.25em}
  \footnotesize
  \centering

  \begin{tabularx}{\textwidth}{ X X r }
    \toprule
    \textbf{Claim} & \textbf{Evidence} & \textbf{Label} \\
    \midrule

    Taking \lexical{antidepressants} is associated with an increase in the A$\beta$ level in the brain of experimental animals. &
    A$\beta$ production in CSF was \numerical{slowed by 37\%} in the \lexical{citalopram} group compared to placebo. &
    \refutes \\
    \midrule

    Radiographic verified pneumonia predictions are improved by the combination of physical examinations with \lexical{C-reactive protein values}. &
    Addition of \lexical{CRP} at the \numerical{optimal cut off of $>$30 mg/L} increased the \numerical{ROC area to 0.77 (0.73 to 0.81)} \dots &
    \supports \\
    \midrule

    \coref{Low saturated fat diets} do not have adverse effects on growth or development of infants. &
    Neurological development of children in the \coref{intervention group} was at least as good as that of children in the control group. &
    \supports \\
    \midrule

    \lexical{Genomic instability} in leukemia cells results from a decrease in reactive oxygen species from oncogene activation. &
     BCR/ABL-induced reactive oxygen species (ROSs) cause \lexical{chronic oxidative DNA damage} \dots &
    \refutes \\

    \bottomrule
  \end{tabularx}

  \caption{Science-specific fact-checking challenges, including recognizing \lexical{lexical relations}, \numerical{quantitative reasoning}, and \coref{coreference}.}
  \label{tbl:scifact_reasoning_types}
\end{table*}
